FedEval: A Holistic Evaluation Framework for Federated Learning

Federated Learning (FL) has been widely accepted as the solution for privacy-preserving machine learning without collecting raw data. While new technologies proposed in the past few years do evolve the FL area, unfortunately, the evaluation results presented in these works fall short in integrity and are hardly comparable because of the inconsistent evaluation metrics and experimental settings. In this paper, we propose a holistic evaluation framework for FL called FedEval, and present a benchmarking study on seven state-of-the-art FL algorithms. Specifically, we first introduce the core evaluation taxonomy model, called FedEval-Core, which covers four essential evaluation aspects for FL: Privacy, Robustness, Effectiveness, and Efficiency, with various well-defined metrics and experimental settings. Based on the FedEval-Core, we further develop an FL evaluation platform with standardized evaluation settings and easy-to-use interfaces. We then provide an in-depth benchmarking study between the seven well-known FL algorithms, including FedSGD, FedAvg, FedProx, FedOpt, FedSTC, SecAgg, and HEAgg. We comprehensively analyze the advantages and disadvantages of these algorithms and further identify the suitable practical scenarios for different algorithms, which is rarely done by prior work. Lastly, we excavate a set of take-away insights and future research directions, which are very helpful for researchers in the FL area.

==> sections/appendices.tex <==
%\section*{Appendix A: Quantifying the Magnitude of Data's Non-IID} \label{appendix:quantifying non-iid}
%
%Assuming we have $K$ clients, and each holds data $x_k \in \mathbb{R}^{n_k \times m}$, where $n_k$ is the number of samples, and $m$ is the number of features. Firstly, we use the histogram to approximate each feature's distribution at each client, and Figure \ref{fig:quantify_noniid_sp} illustrates the histogram results. We use the same number of bins for each feature during the computation, and bin values are normalized such that the sum of all bin values equals 1.
%
%\begin{figure}[h]
%	\centering
%	\includegraphics[scale=0.5]{quantify_noniid_sp.pdf}
%	\caption{Illustration of using histogram to approximate the feature distribution.}
%	\label{fig:quantify_noniid_sp}
%\end{figure}
%
%After the histogram approximate, each client will hold $m$ feature distributions. Then we use Equation \ref{eq:emd} to compute the Wasserstein distance \citep{DBLP:journals/corr/abs-1806-00582} between histograms of the same feature from $client_i$ and $client_j$, where B is the number of bins for the corresponding feature, \highlight{$h_{i,k}$ and $h_{j,k}$ are histogram values of the $k$-t feature (\eg age) from $client_i$ and $client_j$, respectively. For example, if the $k$-th feature is gender, $h_{i,k}=[0.4, 0.6]$ and $h_{j,k}=[0.45, 0.55]$, then $EMD(h_{i,k}, h_{j,k})=0.05+0.05=0.1$.}
%
%\begin{equation} \label{eq:emd}
%	EMD(h_{i,k}, h_{j,k}) = \sum_{b=1}^{B} |h_{i,k}^b - h_{j,k}^b|
%\end{equation}
%
%We use the \highlight{average feature EMD distance} between clients to measure the divergence between their data distribution, and Equation \ref{eq:divergency} shows the detailed computation, \highlight{where m is the total number of features.}
%
%\begin{equation} \label{eq:divergency}
%	D_{i,j} = \frac{1}{m} \sum_{k=1}^m EMD(h_{i,k}, h_{j,k})
%\end{equation}
%
%Finally, we will get a symmetric matrix $D \in \mathbb{R}^{K \times K}$, where $D_{i,j}$ is the distribution divergency between $client_i$ and $client_j$.
%
%\begin{equation} \label{eq:non-iid}
%	\Psi = \frac{1}{K^2} \sum_{i=1}^{K} \sum_{j=1}^{k} D_{i,j}
%\end{equation}
%
%We use the average data distribution divergence between clients to measure the magnitude of data's non-IID, which is denoted as $\Psi$ in Equation \ref{eq:non-iid}.

\section*{Appendix B: Datasets and Parameters} \label{appendix:datasets and parameters}

Following previous work \citep{mcmahan2016communication}, we use $B$, $C$, and $E$ as the parameters of FL mechanisms, $B$ is the local batch size, $C$ is the ratio of clients that participate in each round of training, and $E$ is the number of local training passes (i.e., number of epochs).

\begin{table}
	\centering
	\renewcommand\arraystretch{1.1}
	\setlength{\tabcolsep}{0.3em}
	\caption{Finetuned Hyperparameters}
	\label{tab:dataset}
	\begin{tabular}{ccccc}
		\toprule
		Dataset & \#Device & \#Sample & Model & Parameters \\
		\midrule
		\tabincell{c}{MNIST \\ \citep{lecun1998gradient}} & 100 & 300 & \tabincell{c}{2-layer \\ MLP} & \tabincell{c}{(FedSGD, FedSTC)$\leftarrow$LR=0.5 \\ (FedAvg, FedProx, FedOpt)$\leftarrow$B=16,LR=0.1} \\ \midrule
		\tabincell{c}{FEMNIST \\ \citep{caldas2018leaf}} & 100 & 137 & LeNet & \tabincell{c}{(FedSGD, FedSTC)$\leftarrow$LR=0.1 \\ (FedAvg, FedProx, FedOpt)$\leftarrow$B=8,LR=0.05}  \\ \midrule
		\tabincell{c}{CelebA \\ \citep{caldas2018leaf}} & 100 & 24 & LeNet & \tabincell{c}{(FedSGD, FedSTC)$\leftarrow$LR=0.1 \\ (FedAvg, FedProx, FedOpt)$\leftarrow$B=4,LR=0.05} \\ \midrule
		\tabincell{c}{Sent140 \\ \citep{go2009twitter}} & 100 & 140 & \tabincell{c}{2-layer \\ LSTM} & \tabincell{c}{(FedSGD, FedSTC)$\leftarrow$LR=0.05 \\ (FedAvg, FedProx, FedOpt)$\leftarrow$B=4,LR=0.0001} \\
		\bottomrule
	\end{tabular}
\end{table}

\Cref{tab:dataset} shows the four benchmarking datasets that we used in the experiments, and the corresponding finetuned parameters. We use 100 clients in all the experiments. We set $B=\infty,C=1$, and $E=1$ for FedSGD, empirically chose B and E for FdAvg, then perform a fine-grained search on learning rates from $0.0001 \sim 1.0$. The best hyperparameters are shown in \Cref{tab:dataset}. The parameter-searching results (e.g., tuning learning rates) are presented in the appendix \ref{appendix:params_tune}. For datasets that are not collected in FL style (e.g., MNIST), we simulate the non-IID data by restricting the number of clients' local image classes. For example, The experiments of clients have 1 class of MNIST images are reported in robustness benchmarks. For datasets collected in FL manner (i.e., the samples are organized by who generated them), we partition the data naturally based on the identity and randomly shuffle the data between clients to create an ideal IID data setting. To simplify the comparison, we only present the non-IID data results in the robustness evaluation and use the IID setting in other experiments.

All the experiments run on a Linux server \highlight{with Ubuntu 18.04 installed, Intel(R) i7-9700KF} 8-core 3.7GHz CPU, 128GB RAM, \highlight{960G SSD storage}. \highlight{All the experiments are performed using FedEval (\url{https://github.com/Di-Chai/FedEval}), which is a benchmarking system maintained by us. All the parties are simulated using docker containers, which are connected using docker network using the bridge mode.} We limit the clients' bandwidth to 100Mb/s and do not restrict the server's bandwidth. We set the network latency to 50ms. \highlight{The reproduction guideline is provided at \url{https://di-chai.github.io/FedEval/Reproduce.html}, and the benchmarking results are also available online at \url{https://di-chai.github.io/FedEval/BenchmarkResults.html}}.

%\section{Homepages of existing federated learning frameworks} \label{appendix:homepage}
%
%\begin{itemize}
%	\item TFF \cite{tensorflow2019federated}: \url{https://www.tensorflow.org/federated}
%	\item FATE \cite{yang2019federated}: \url{https://github.com/FederatedAI/FATE}
%	\item PaddleFL \cite{ma2019paddlepaddle}: \url{https://github.com/PaddlePaddle/PaddleFL}
%	\item LEAF \cite{caldas2018leaf}: \url{https://github.com/TalwalkarLab/leaf}
%	\item PySyft \cite{ryffel2018generic}: \url{https://github.com/OpenMined/PySyft}
%	\item FedML \cite{he2020fedml}: \url{https://github.com/FedML-AI/FedML}
%\end{itemize}

%\section*{Appendix C: Parameter Tuning results} \label{appendix:params_tune}
%
%\Cref{tab:parameter_tune} shows the results of tuning the learning rates (LR), and the best parameters are bolded. \highlight{Since the LR tuning is costly in time, we first partition the models into groups and do the parameter tuning for only one model in each group. FedSTC and FedSGD require all the parties to join the model training in each round. Thus we only tune LR for FedSGD, and FedSTC inherits the best LR from FedSGD. FedProx, FedOpt, and FedAvg select a subset of the parties during each round of training. Thus we only tune LR for FedAvg, then FedProx and FedOpt inherit the best LR.}
%
%\vspace{-2mm}
%\begin{table}
%	\centering
%	\renewcommand\arraystretch{0.5}
%	\caption{Results of tuning the learning rates. \highlight{Total time is in minutes.}}
%	\label{tab:parameter_tune}
%	\begin{tabular}{c|c|c|c|c|ccc}
%		\toprule
%		dataset & B & C & E & lr & \highlight{FL Effectiveness} & total\_time & total\_rounds \\
%		\midrule
%		celeba & 4 & 0.1 & 10 & 0.0001 & 0.83778 & 68.49028  & 1776.41667 \\
%		celeba & 4 & 0.1 & 10 & 0.0005 & 0.84639 & 24.57500 & 633.58333 \\
%		celeba & 4 & 0.1 & 10 & 0.001 & 0.85545 & 17.58485 & 451.09091 \\
%		celeba & 4 & 0.1 & 10 & 0.005 & 0.85970 & 11.30909 & 288.00000  \\
%		celeba & 4 & 0.1 & 10 & 0.01 & 0.86515 & 9.38182 & 238.72727  \\
%		celeba & 4 & 0.1 & 10 & \textbf{0.05} & 0.88455 & 7.57273 & 190.45455  \\
%		celeba & 4 & 0.1 & 10 & 0.1 & 0.84212 & 6.98636 & 175.81818  \\
%		celeba & 4 & 0.1 & 10 & 0.5 & 0.51970 & 7.25303 & 183.09091  \\
%		celeba & 4 & 0.1 & 10 & 1 & 0.53000 & 5.65758 & 141.63636  \\
%		\midrule
%		celeba & 1000 & 1 & 1 & 0.0001 & 0.54933 & 182.82500  & 2738.50000 \\
%		celeba & 1000 & 1 & 1 & 0.0005 & 0.61767 & 200.22333 & 3000.00000 \\
%		celeba & 1000 & 1 & 1 & 0.001 & 0.65900 & 161.47333  & 2420.000001 \\
%		celeba & 1000 & 1 & 1 & 0.005 & 0.86300 & 177.60333  & 2667.70000 \\
%		celeba & 1000 & 1 & 1 & 0.01 & 0.85200 & 97.45667  & 1465.80000 \\
%		celeba & 1000 & 1 & 1 & 0.05 & 0.85900 & 33.68167 & 505.20000  \\
%		celeba & 1000 & 1 & 1 & \textbf{0.1} & 0.87367 & 31.38000 & 470.90000  \\
%		celeba & 1000 & 1 & 1 & 0.5 & 0.62367 & 12.48667 & 186.20000  \\
%		celeba & 1000 & 1 & 1 & 1 & 0.56433 & 10.21000 & 152.60000  \\
%		\midrule
%		femnist & 8 & 0.1 & 10 & 0.0001 & 0.78523 & 137.64000 & 3000.00000 \\
%		femnist & 8 & 0.1 & 10 & 0.0005 & 0.82746 & 54.82500 & 1189.30000 \\
%		femnist & 8 & 0.1 & 10 & 0.001 & 0.82451 & 34.11833 & 740.20000 \\
%		femnist & 8 & 0.1 & 10 & 0.005 & 0.84525 & 23.28833 & 503.20000 \\
%		femnist & 8 & 0.1 & 10 & 0.01 & 0.85655 & 19.94333 & 431.00000  \\
%		femnist & 8 & 0.1 & 10 & \textbf{0.05} & 0.85202 & 13.00833 & 243.91667  \\
%		femnist & 8 & 0.1 & 10 & 0.1 & 0.84469 & 11.06667 & 238.70000  \\
%		femnist & 8 & 0.1 & 10 & 0.5 & 0.07335 & 6.86833 & 146.30000  \\
%		femnist & 8 & 0.1 & 10 & 1 & 0.07260 & 9.77167 & 209.60000  \\
%		\midrule
%		femnist & 1000 & 1 & 1 & 0.0001 & 0.04994 & 162.27167 & 3000.00000 \\
%		femnist & 1000 & 1 & 1 & 0.0005 & 0.10840 & 161.82667 & 3000.00000 \\
%		femnist & 1000 & 1 & 1 & 0.001 & 0.13685 & 161.88667 & 3000.00000 \\
%		femnist & 1000 & 1 & 1 & 0.005 & 0.59363 & 161.99167 & 3000.00000 \\
%		femnist & 1000 & 1 & 1 & 0.01 & 0.71425 & 162.06167 & 3000.00000 \\
%		femnist & 1000 & 1 & 1 & 0.05 & 0.84757 & 114.91000  & 2129.00000 \\
%		femnist & 1000 & 1 & 1 & \textbf{0.1} & 0.85556 & 77.66333  & 1435.80000 \\
%		femnist & 1000 & 1 & 1 & 0.5 & 0.18482 & 9.29167 & 172.80000  \\
%		femnist & 1000 & 1 & 1 & 1 & 0.10863 & 9.84167 & 182.30000  \\
%		\midrule
%		mnist & 16 & 0.1 & 10 & 0.0001 & 0.95967 & 208.07917 & 3000.00000 \\
%		mnist & 16 & 0.1 & 10 & 0.0005 & 0.97689 & 207.40000 & 3000.00000 \\
%		mnist & 16 & 0.1 & 10 & 0.001 & 0.97967 & 151.70000 & 2189.33333 \\
%		mnist & 16 & 0.1 & 10 & 0.005 & 0.97818 & 43.05128 & 622.92308  \\
%		mnist & 16 & 0.1 & 10 & 0.01 & 0.97903 & 37.92821 & 548.84615  \\
%		mnist & 16 & 0.1 & 10 & 0.05 & 0.98136 & 22.68590 & 327.38462  \\
%		mnist & 16 & 0.1 & 10 & \textbf{0.1} & 0.98282 & 17.71795 & 255.92308  \\
%		mnist & 16 & 0.1 & 10 & 0.5 & 0.98176 & 11.53636 & 166.18182  \\
%		mnist & 16 & 0.1 & 10 & 1 & 0.10267 & 7.09697 & 102.00000 \\
%		\midrule
%		mnist & 1000 & 1 & 1 & 0.0001 & 0.47825 & 468.54583 & 3000.00000 \\
%		mnist & 1000 & 1 & 1 & 0.0005 & 0.84633 & 470.17917 & 3000.00000 \\
%		mnist & 1000 & 1 & 1 & 0.001 & 0.90056 & 465.70556 & 3000.00000 \\
%		mnist & 1000 & 1 & 1 & 0.005 & 0.94311 & 464.52778 & 3000.00000 \\
%		mnist & 1000 & 1 & 1 & 0.01 & 0.95444 & 463.28333 & 3000.00000 \\
%		mnist & 1000 & 1 & 1 & 0.05 & 0.97300 & 470.60000 & 3000.00000 \\
%		mnist & 1000 & 1 & 1 & 0.1 & 0.97967 & 471.68889 & 3000.00000 \\
%		mnist & 1000 & 1 & 1 & \textbf{0.5} & 0.98185 & 144.75000 & 922.77778  \\
%		mnist & 1000 & 1 & 1 & 1 & 0.97983 & 79.25625  & 507.75000 \\
%		\midrule
%		sentiment140 & 4 & 0.1 & 10 & \textbf{0.0001} & 0.76704 & 573.85167  & 2889.80000 \\
%		sentiment140 & 4 & 0.1 & 10 & 0.0005 & 0.76427 & 211.73667  & 1031.20000  \\
%		sentiment140 & 4 & 0.1 & 10 & 0.001 & 0.75777 & 163.46000  & 789.00000  \\
%		sentiment140 & 4 & 0.1 & 10 & 0.005 & 0.75563 & 128.86167 & 160.10000 \\
%		sentiment140 & 4 & 0.1 & 10 & 0.01 & 0.74879 & 104.56667 & 128.70000 \\
%		sentiment140 & 4 & 0.1 & 10 & 0.05 & 0.70871 & 86.20833 & 105.00000 \\
%		sentiment140 & 4 & 0.1 & 10 & 0.1 & 0.68279 & 83.35000 & 103.00000 \\
%		sentiment140 & 4 & 0.1 & 10 & 0.5 & 0.66621 & 83.36667 & 102.00000 \\
%		sentiment140 & 4 & 0.1 & 10 & 1 & 0.65584 & 84.31667 & 104.00000 \\
%		\midrule
%		sentiment140 & 1000 & 1 & 1 & 0.0001 & 0.65377 & 869.46667 & 3000.00000 \\
%		sentiment140 & 1000 & 1 & 1 & 0.005 & 0.74534 & 655.61667  & 9351.00000 \\
%		sentiment140 & 1000 & 1 & 1 & 0.01 & 0.76434 & 700.50833 & 10000.00000 \\
%		sentiment140 & 1000 & 1 & 1 & \textbf{0.05} & 0.77436 & 351.05000  & 4973.50000 \\
%		sentiment140 & 1000 & 1 & 1 & 0.1 & 0.76766 & 257.91667  & 3445.60000 \\
%		sentiment140 & 1000 & 1 & 1 & 0.5 & 0.71942 & 137.35000  & 472.66667 \\
%		sentiment140 & 1000 & 1 & 1 & 1 & 0.71297 & 146.77222  & 505.33333 \\
%		\bottomrule
%	\end{tabular}
%\end{table}


